AutoInit: Analytic Signal-Preserving Weight Initialization for Neural Networks

Neural networks require careful weight initialization to prevent signals from exploding or vanishing. Existing initialization schemes solve this problem in specific cases by assuming that the network has a certain activation function or topology. It is difficult to derive such weight initialization strategies, and modern architectures therefore often use these same initialization schemes even though their assumptions do not hold. This paper introduces AutoInit, a weight initialization algorithm that automatically adapts to different neural network architectures. By analytically tracking the mean and variance of signals as they propagate through the network, AutoInit appropriately scales the weights at each layer to avoid exploding or vanishing signals. Experiments demonstrate that AutoInit improves performance of convolutional, residual, and transformer networks across a range of activation function, dropout, weight decay, learning rate, and normalizer settings, and does so more reliably than data-dependent initialization methods. This flexibility allows AutoInit to initialize models for everything from small tabular tasks to large datasets such as ImageNet. Such generality turns out particularly useful in neural architecture search and in activation function discovery. In these settings, AutoInit initializes each candidate appropriately, making performance evaluations more accurate. AutoInit thus serves as an automatic configuration tool that makes design of new neural network architectures more robust. The AutoInit package provides a wrapper around TensorFlow models and is available at https://github.com/cognizant-ai-labs/autoinit.

==> figures/afn_plots.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{plots/afn_plots.pdf}\\[2em]
    \includegraphics[width=\linewidth]{plots/zero_gaussian_mean_afn_plots.pdf}
 \caption{A representative sample of top-performing activation functions from the PANGAEA search space.  Each plot is titled with the function definition and the accuracy achieved when paired with All-CNN-C initialized with AutoInit or AutoInit++.  Some activation functions are fixed, while others have learnable parameters $\alpha$, $\beta$, and $\gamma$.  AutoInit is compatible with both types of functions.  For the parametric ones, the red line shows the activation function at initialization, with $\alpha = \beta = \gamma = 1$.  The blue lines show the shapes the activation function takes during training, created by sampling values for the learnable parameters from $\mathcal{U}(0.5, 2.0)$.  By achieving good performance with all of these functions, AutoInit demonstrates flexibility that should turn out useful for developing new activation functions in the future.}
    \label{fig:afn_plots}
\end{figure}
% functional duplicates removed


==> figures/allcnnc_activation_fn.tex <==
\begin{table}
    \centering
    \begin{tabular}{lll}
        \toprule
        Activation & Glorot Uniform & AutoInit \\ 
        \midrule
        ELU & 89.53 & 89.69 {\color{ForestGreen} \scriptsize (+0.16)} \\
        GELU & 89.81 & 89.90 {\color{ForestGreen} \scriptsize (+0.09)} \\
        ReLU & 89.10 & 89.98 {\color{ForestGreen} \scriptsize (+0.88)} \\
        SELU & 90.06 & 90.02 {\color{OrangeRed} \scriptsize (-0.04)} \\
        Softplus & 10.00 & 87.83 {\color{ForestGreen} \scriptsize (+77.83)} \\
        Softsign & 52.60 & 59.59 {\color{ForestGreen} \scriptsize (+6.99)} \\
        Swish & 89.67 & 89.46 {\color{OrangeRed} \scriptsize (-0.21)} \\
        tanh & 71.28 & 73.36 {\color{ForestGreen} \scriptsize (+2.08)} \\
        \bottomrule
    \end{tabular}
    \caption{All-CNN-C test accuracy on CIFAR-10 with different activation functions and weight initialization strategies.  Results are shown as the median of three independent runs.  AutoInit stabilizes training by adapting to each activation function.}
    \label{tab:allcnnc_activation_fn}
\end{table}

==> figures/allcnnc_dropout.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{lll}
%         \toprule
%         Dropout Rate & Default Init & AutoInit \\ 
%         \midrule
%         0.0 (no dropout) & 89.13 & 89.68 {\color{ForestGreen} \scriptsize (+0.55)} \\
%         0.1 & 88.51 & 90.22 {\color{ForestGreen} \scriptsize (+1.71)} \\
%         0.2 & 88.91 & 89.76 {\color{ForestGreen} \scriptsize (+0.85)} \\
%         0.3 & 89.45 & 89.77 {\color{ForestGreen} \scriptsize (+0.32)} \\
%         0.4 & 88.25 & 89.93 {\color{ForestGreen} \scriptsize (+1.68)} \\
%         0.5 (default setting) & 89.10 & 89.98 {\color{ForestGreen} \scriptsize (+0.88)} \\
%         0.6 & 87.28 & 89.99 {\color{ForestGreen} \scriptsize (+2.71)} \\
%         0.7 & 88.61 & 89.50 {\color{ForestGreen} \scriptsize (+0.89)} \\
%         0.8 & 86.55 & 88.95 {\color{ForestGreen} \scriptsize (+2.40)} \\
%         0.9 & 84.41 & 85.64 {\color{ForestGreen} \scriptsize (+1.23)} \\
%         \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:allcnnc_dropout}
% \end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{plots/allcnnc_dropout.pdf}
    \caption{All-CNN-C test accuracy on CIFAR-10 with different dropout rates and weight initialization strategies.  Each result is from a single run.  AutoInit improves accuracy in every case and gets good performance with a wider range of dropout values compared to the default initialization.}
    \label{fig:allcnnc_dropout}
\end{figure}

==> figures/allcnnc_l2_penalty.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{lll}
%         \toprule
%         L2 Penalty & Default Init & AutoInit \\ 
%         \midrule
%         0 & 88.93 & 90.20 {\color{ForestGreen} \scriptsize (+1.27)} \\
%         0.00001 & 91.91 & 92.25 {\color{ForestGreen} \scriptsize (+0.34)} \\
%         0.0001 & 92.17 & 92.67 {\color{ForestGreen} \scriptsize (+0.50)} \\
%         0.001 (default) & 89.10 & 89.98 {\color{ForestGreen} \scriptsize (+0.88)} \\
%         0.01 & 10.00 & 47.91 {\color{ForestGreen} \scriptsize (+37.91)} \\
%         \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:allcnnc_l2_penalty}
% \end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{plots/allcnnc_l2_penalty.pdf}
    \caption{All-CNN-C test accuracy on CIFAR-10 with different weight decay settings and weight initialization strategies.  Each result is from a single run.  AutoInit outperforms the default strategy in every case.}
    \label{fig:allcnnc_l2_penalty}
\end{figure}


==> figures/allcnnc_lr_scale.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{lll}
%         \toprule
%         LR Scale & Default Init & AutoInit \\ 
%         \midrule
%         0.1 & 78.57 & 85.06 {\color{ForestGreen} \scriptsize (+6.49)} \\
%         0.2 & 83.78 & 87.21 {\color{ForestGreen} \scriptsize (+3.43)} \\
%         0.5 & 85.53 & 89.39 {\color{ForestGreen} \scriptsize (+3.86)} \\
%         1 & 89.10 & 89.98 {\color{ForestGreen} \scriptsize (+0.88)} \\
%         2 & 90.15 & 90.13 {\color{OrangeRed} \scriptsize (-0.02)} \\
%         5 & 89.31 & 89.24 {\color{OrangeRed} \scriptsize (-0.07)} \\
%         10 & 11.22 & 15.36 {\color{ForestGreen} \scriptsize (+4.14)} \\
%         \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:allcnnc_lr_scale}
% \end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{plots/allcnnc_lr_multiplier.pdf}
    \caption{All-CNN-C test accuracy on CIFAR-10 with different learning rate schedule multipliers and weight initialization strategies.  Each result is from a single run.  AutoInit is comparable to or outperforms the default initialization strategy in every case.  AutoInit also achieves good performance with a broader range of learning rate schedules compared to the default strategy.}
    \label{fig:allcnnc_lr_scale}
\end{figure}

==> figures/codeepneat.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{plots/codeepneat.pdf}
    \caption{The CoDeepNEAT method.  Modules (middle) replace the nodes in the blueprint (left) to create a candidate neural network (right).  CoDeepNEAT produces a variety of network architectures, which then provide a comprehensive evaluation of the generality of AutoInit.}
    % \caption{The CoDeepNEAT method for coevolving populations of modules and blueprints.  The modules (middle) replace the nodes in the blueprint (left) to create a candidate neural network (right).  Each module species is evolved separately, and each node in the blueprint specifies the species from which the module is drawn to replace it. CoDeepNEAT produces a variety of network architectures, which then provide a comprehensive evaluation of the generality of AutoInit.}
    \label{fig:codeepneat}
\end{figure}

==> figures/evolved_models.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=0.33\linewidth]{network_visualizations/mnist.pdf} \\
    \textbf{MNIST} \\[2em]
    \includegraphics[width=0.33\linewidth]{network_visualizations/pmlb.pdf} \\
    \textbf{PMLB Adult} \\[2em]
    \includegraphics[width=0.33\linewidth]{network_visualizations/textclassifier.pdf} \\
    \textbf{Wikipedia Toxicity}
    \caption{Three representative networks evolved with AutoInit for the MNIST, PMLB Adult, and Wikipedia Toxicity tasks.  Although the networks are distinctly different from current models in the literature, AutoInit is able to initialize them properly, leading to good performance in each case. }
    \label{fig:evolved_models}
\end{figure*}



==> figures/pangaea.tex <==

\usetikzlibrary{shapes.geometric, arrows, positioning, calc}
\tikzstyle{input} = [rectangle, rounded corners, text centered, draw=black, fill=red!30]
\tikzstyle{unary} = [rectangle, rounded corners, text centered, draw=black, fill=yellow!30]
\tikzstyle{binary} = [rectangle, rounded corners, text centered, draw=black, fill=blue!30]
\tikzstyle{arrow} = [thick, ->,>=stealth]
\tikzstyle{output} = [rectangle, rounded corners, text centered, draw=black, fill=green!30]
\tikzstyle{invisible} = [rectangle, text centered]
\tikzstyle{maybeparam} = [draw, circle, dashed, fill=cyan!30]

\begin{figure*}
    \centering
    \begin{adjustbox}{max width=\linewidth}
        {\renewcommand{\arraystretch}{2}%
        \begin{tabular}{c@{\hskip 3em}c@{\hskip 3em}c@{\hskip 3em}c}
            {\renewcommand{\arraystretch}{1}%
            \begin{tabular}{llll} 
                \toprule 
                \multicolumn{3}{c}{\textbf{Unary}} & \multicolumn{1}{l}{\textbf{Binary}} \\ \midrule
                $0$                & $e^x-1$               & $\textrm{ReLU}(x)$        & $x_1 + x_2$ \\
                $1$                & $\log(\sigma(x))$     & $\textrm{ELU}(x)$         & $x_1 - x_2$ \\
                $x$                & $\textrm{erf}(x)$     & $\textrm{SELU}(x)$        & $x_1 \cdot x_2$ \\
                $-x$               & $\textrm{erfc}(x)$    & $\textrm{Swish}(x)$       & $x_1 / x_2$ \\
                $|x|$              & $\textrm{sinh}(x)$    & $\textrm{Softplus}(x)$    & $x_1^{x_2}$ \\
                $x^{-1}$           & $\textrm{cosh}(x)$    & $\textrm{Softsign}(x)$    & $\max\{x_1, x_2\}$ \\
                $x^2$              & $\textrm{tanh}(x)$    & $\textrm{HardSigmoid}(x)$ & $\min\{x_1, x_2\}$\\
                $e^x$              & $\textrm{arcsinh}(x)$ & $\textrm{bessel\_i0e}(x)$ & \\
                $\sigma(x)$        & $\textrm{arctan}(x)$  & $\textrm{bessel\_i1e}(x)$ & \\

                
                \bottomrule
            \end{tabular}}

            &
            
            \begin{tikzpicture}[node distance=3em, baseline=-4.5em]
            
                \node (output2) [output] {$f(x)$};
                \node (unary4) [unary, below of=output2] {Unary};
                \node (unary3) [unary, below of=unary4] {Unary};
                \node (input3) [input, below of=unary3] {$x$};
                
                \draw [arrow] (input3) -- (unary3);
                \draw [arrow] (unary3) -- (unary4);
                \draw [arrow] (unary4) -- (output2);
            
                \node (output) [output, right of=output2, xshift=4em] {$f(x)$};
                \node (binary) [binary, below of=output] {Binary};
                \node (unary1) [unary, below of=binary, xshift=-2em] {Unary};
                \node (unary2) [unary, below of=binary, xshift=2em] {Unary};
                \node (input1) [input, below of=unary1] {$x$};
                \node (input2) [input, below of=unary2] {$x$};
                
                \draw [arrow] (input1) -- (unary1);
                \draw [arrow] (input2) -- (unary2);
                \draw [arrow] (unary1) -- (binary);
                \draw [arrow] (unary2) -- (binary);
                \draw [arrow] (binary) -- (output);

            \end{tikzpicture}
            &
            \begin{tabular}{cccccccc}
     
                \begin{tikzpicture}[node distance=3em]
        
                    \node [output] (out1) {$f(x)$};
                    \node [unary, below of=out1] (u1) {$x^2$};
                    \node [binary, below of=u1] (b1) {$x_1 + x_2$};
                    \node [unary, below of=b1, xshift=-2em] (u2) {$\textrm{tanh}(x)$};
                    \node [unary, below of=b1, xshift=2em] (u3) {$|x|$};
                    \node [unary, below of=u3] (u4) {$\textrm{erf}(x)$};
                    \node [input, below of=u4] (i1) {$x$};
                    \node [input, left of=i1, xshift=-1em] (i2) {$x$};
                    
                    \node [invisible, below of=out1, yshift=-14em] (d) {\normalsize Parent};
                    
                    \draw [arrow] (i1) -- (u4);
                    \draw [arrow] (i2) -- (u2);
                    \draw [arrow] (u4) -- (u3);
                    \draw [arrow] (u3) -- (b1);
                    \draw [arrow] (u2) -- (b1);
                    \draw [arrow] (b1) -- (u1);
                    \draw [arrow] (u1) -- (out1);
                
                \end{tikzpicture}
                &
                \begin{tikzpicture}[node distance=3em]
                
                    \node [output] (out1) {$f(x)$};
                    \node [unary, below of=out1] (u1) {$x^2$};
                    \node [binary, below of=u1] (b1) {$x_1 + x_2$};
                    \node [unary, below of=b1, xshift=-2em, draw=red, line width=1] (swish) {$\textrm{Swish}(x)$};
                    \node [unary, below of=swish] (u2) {$\textrm{tanh}(x)$};
                    \node [unary, below of=b1, xshift=2em] (u3) {$|x|$};
                    \node [unary, below of=u3] (u4) {$\textrm{erf}(x)$};
                    \node [input, below of=u4] (i1) {$x$};
                    \node [input, left of=i1, xshift=-1em] (i2) {$x$};
                    
                    \node [invisible, below of=out1, yshift=-14em] (d) {\normalsize Insert};
                    
                    \draw [arrow] (i1) -- (u4);
                    \draw [arrow] (i2) -- (u2);
                    \draw [arrow] (u4) -- (u3);
                    \draw [arrow] (u3) -- (b1);
                    \draw [arrow] (u2) -- (swish);
                    \draw [arrow] (swish) -- (b1);
                    \draw [arrow] (b1) -- (u1);
                    \draw [arrow] (u1) -- (out1);
                
                \end{tikzpicture}
                &
                \begin{tikzpicture}[node distance=3em]
                
                    \node [output] (out1) {$f(x)$};
                    \node [unary, below of=out1] (u1) {$x^2$};
                    \node [unary, below of=u1] (u3) {$|x|$};
                    \node [unary, below of=u3] (u4) {$\textrm{erf}(x)$};
                    \node [input, below of=u4] (i1) {$x$};
                    
                    \node [invisible, below of=out1, yshift=-14em] (d) {\normalsize Remove};
                    
                    \draw [arrow] (i1) -- (u4);
                    \draw [arrow] (u4) -- (u3);
                    \draw [arrow, draw=red] (u3) -- (u1);
                    \draw [arrow] (u1) -- (out1);
                
                \end{tikzpicture}
                &
                \begin{tikzpicture}[node distance=3em]
                
                    \node [output] (out1) {$f(x)$};
                    \node [unary, below of=out1] (u1) {$x^2$};
                    \node [binary, below of=u1, draw=red, line width=1] (b1) {$x_1 \cdot x_2$};
                    \node [unary, below of=b1, xshift=-2em] (u2) {$\textrm{tanh}(x)$};
                    \node [unary, below of=b1, xshift=2em] (u3) {$|x|$};
                    \node [unary, below of=u3] (u4) {$\textrm{erf}(x)$};
                    \node [input, below of=u4] (i1) {$x$};
                    \node [input, left of=i1, xshift=-1em] (i2) {$x$};
                    
                    \node [invisible, below of=out1, yshift=-14em] (d) {\normalsize Change};
                    
                    \draw [arrow] (i1) -- (u4);
                    \draw [arrow] (i2) -- (u2);
                    \draw [arrow] (u4) -- (u3);
                    \draw [arrow] (u3) -- (b1);
                    \draw [arrow] (u2) -- (b1);
                    \draw [arrow] (b1) -- (u1);
                    \draw [arrow] (u1) -- (out1);
                
                \end{tikzpicture}
                &
                \begin{tikzpicture}[node distance=3em]
                
                    \node [output] (out1) {$f(x)$};
                    \node [unary, below of=out1, draw=red, line width=1] (u1) {$-x$};
                    \node [binary, below of=u1, draw=red, line width=1] (b1) {$\max\{x_1, x_2\}$};
                    \node [unary, below of=b1, xshift=-2em, draw=red, line width=1] (u2) {$0$};
                    \node [unary, below of=b1, xshift=2em, draw=red, line width=1] (u3) {$\textrm{tanh}(x)$};
                    \node [unary, below of=u3, draw=red, line width=1] (u4) {$\textrm{SELU}(x)$};
                    \node [input, below of=u4] (i1) {$x$};
                    \node [input, left of=i1, xshift=-1em] (i2) {$x$};
                    
                    \node [invisible, below of=out1, yshift=-14em] (d) {\normalsize Regenerate};
                    
                    \draw [arrow] (i1) -- (u4);
                    \draw [arrow] (i2) -- (u2);
                    \draw [arrow] (u4) -- (u3);
                    \draw [arrow] (u3) -- (b1);
                    \draw [arrow] (u2) -- (b1);
                    \draw [arrow] (b1) -- (u1);
                    \draw [arrow] (u1) -- (out1);
                
                \end{tikzpicture}
            \end{tabular}
            &
            \begin{tabular}{cc}            
                \begin{tikzpicture}[node distance=3em]
                
                    \node (output) [output] {$f(x)$};
                    \node (unary) [unary, below of=output] {$\sigma(x)$};
                    \node (binary) [binary, below of=unary] {$x_1 - x_2$};
                    \node (unary1) [unary, below of=binary, xshift=-2em] {$|x|$};
                    \node (unary2) [unary, below of=binary, xshift=2em] {$\textrm{arctan}(x)$};
                    \node (input1) [input, below of=unary1] {$x$};
                    \node (input2) [input, below of=unary2] {$x$};
            
                    \draw [arrow] (input1) -- (unary1);
                    \draw [arrow, draw=red] (input2) -- (unary2);
                    \draw [arrow, draw=red] (unary1) -- (binary);
                    \draw [arrow] (unary2) -- (binary);
                    \draw [arrow] (binary) -- (unary);
                    \draw [arrow, draw=red] (unary) -- (output);
                    
                \end{tikzpicture}
                &
                \begin{tikzpicture}[node distance=3em]
        
                    \node (output) [output] {$f(x)$};
                    \node (p1) [maybeparam, below of=output] {$\alpha$};
                    \node (unary) [unary, below of=p1] {$\sigma(x)$};
                    \node (binary) [binary, below of=unary] {$x_1 - x_2$};
                    \node (p5) [maybeparam, below of=binary, xshift=-2em] {$\beta$};
                    \node (unary1) [unary, below of=p5] {$|x|$};
                    \node (unary2) [unary, below of=binary, xshift=2em] {$\textrm{arctan}(x)$};
                    \node (p4) [maybeparam, below of=unary2] {$\gamma$};
                    \node (input1) [input, below of=unary1] {$x$};
                    \node (input2) [input, below of=p4] {$x$};
                    
            
                    \draw [arrow] (input1) -- (unary1);
                    \draw [arrow] (input2) -- (p4);
                    \draw [arrow] (p4) -- (unary2); 
                    \draw [arrow] (unary1) -- (p5);
                    \draw [arrow] (p5) -- (binary);
                    \draw [arrow] (unary2) -- (binary);
                    \draw [arrow] (binary) -- (unary);
                    \draw [arrow] (unary) -- (p1);
                    \draw [arrow] (p1) -- (output);
                    
                \end{tikzpicture}
            \end{tabular}
            \\
            {\LARGE \textbf{(a) Search Space}}
            &
            {\LARGE \textbf{(b) Initialization}}
            &
            {\LARGE \textbf{(c) Mutation}}
            &
            {\LARGE \textbf{(d) Parameterization}}
            
        \end{tabular}}
    \end{adjustbox}
    \caption{The PANGAEA method \cite{bingham2020discovering} for representing activation functions.  (a) \textbf{Search Space:} Activation functions are represented as computation graphs composed of unary and binary operators.   (b) \textbf{Initialization: }A randomly created activation function has one of two possible functional forms: either $f(x) = \texttt{unary1}(\texttt{unary2}(x))$ or $f(x) = \texttt{binary}(\texttt{unary1}(x), \texttt{unary2}(x))$.   (c) \textbf{Mutation:} Randomly selected mutations modify the original parent activation function.   (d) \textbf{Parameterization:} Up to three learnable parameters are added to the activation function in order to allow the function's shape to be fine-tuned via gradient descent.  For example, the rightmost computation graph represents the parametric activation function $f(x) = \alpha \cdot \sigma (\beta \cdot | x | - \arctan ( \gamma \cdot x ) )$. In this manner, PANGAEA generates a variety of activation functions that can be used to evaluate AutoInit's generality and flexibility.}
    \label{fig:pangaea}
\end{figure*}


==> figures/resnet_vary_lr.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth]{plots/resnet_vary_lr.pdf}
    \includegraphics[width=0.49\linewidth]{plots/resnet_vary_lr_no_bn.pdf}
    \caption{ResNet-164 test accuracy on CIFAR-10 with a variety of learning rate schedules and weight initializations.  Results are from a single run.  AutoInit is comparable to or outperforms the default initialization in every case.}
    \label{fig:resnet_vary_lr}
\end{figure}

==> figures/signal_propagation_afn.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{plots/signal_propagation_vary_afn.pdf}
    \caption{Signal propagation across All-CNN-C networks with different activation functions.  Gaussian input was propagated through the networks and the empirical variance computed at each layer.  The variance naturally fluctuates as each layer modifies its input.  At layers with weights (highlighted in red), AutoInit scales the weights appropriately to return the variance to approximately 1.0.}
    \label{fig:signal_propagation_afn}
\end{figure}

==> figures/signal_propagation_dropout.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{plots/signal_propagation_vary_dropout.pdf}
    % \includegraphics[width=0.49\linewidth]{plots/signal_propagation_vary_dropout_default.pdf}
    % \includegraphics[width=0.49\linewidth]{plots/signal_propagation_vary_dropout_autoinit.pdf}
    \caption{Signal propagation in All-CNN-C networks with different dropout rates.  The plots were created by feeding Gaussian inputs to the network and computing the empirical variance at each layer.  GAP2D refers to a \texttt{GlobalAveragePooling2D} layer. With the default initialization, signal variance vanishes with depth, and the behavior is different with each dropout rate.  With AutoInit, the signal variance remains approximately constant at 1.0 after each layer with initializable weights (highlighted in red).  The variance is consistent across the network regardless of the dropout rate.}
    \label{fig:signal_propagation_dropout}
\end{figure}

==> figures/usage.tex <==
\begin{figure}
    \centering
    \begin{verbatim}
        # Install
        pip install git+https://github.com/~~~ANONYMIZED~~~/
        
        # Import
        from autoinit.initializer.initalize_weights import AutoInit
        
        # Initialize
        model = AutoInit().initialize_model(model)
    \end{verbatim}
    \caption{The AutoInit package provides a wrapper around TensorFlow models.}
    \label{fig:usage}
\end{figure}

% TODO
% Update code with latest ENN changes
% Change name from universal to autoinit


==> sections/appendices.tex <==
\section*{Appendices}
The following appendices can be found online at \url{https://arxiv.org/abs/2109.08958}.
\begin{itemize}
    \item[A:] Mean and Variance Estimation for Different Layer Types
    \item[B:] Convolutional, Residual, and Transformer Network Experiment Details
    \item[C:] Neural Architecture Search Experiment Details
    \item[D:] Statistical Significance of Results in Activation Function Meta-Learning
    \item[E:] Future Work
    \item[F:] Computing Infrastructure
\end{itemize}
In particular, Appendix \ref{sec:mean_variance_estimation} contains mean and variance mapping functions $g$ for the following layer types:


{\small
\noindent\textbf{Weights } \texttt{Conv\{1D,2D,3D\}}, \texttt{DepthwiseConv\{1D,2D\}}, \texttt{Dense}

\noindent\textbf{Activation Functions } \texttt{Activation}, \texttt{elu}, \texttt{expo\-nen\-tial}, \texttt{gelu}, \texttt{hard\_sigmoid}, \texttt{LeakyReLU}, \texttt{linear}, \texttt{PReLU}, \texttt{ReLU}, \texttt{selu}, \texttt{sigmoid}, \texttt{softplus}, \texttt{softsign}, \texttt{swish}, \texttt{tanh}, \texttt{ThresholdedReLU}

\noindent\textbf{Dropout } \texttt{SpatialDropout\{1D,2D,3D\}}, \texttt{Dropout}

\noindent\textbf{Pooling } \texttt{AveragePooling\{1D,2D,3D\}}, \texttt{MaxPooling\{1D,\allowbreak2D,3D\}},  \texttt{Global\-Average\-Pooling\{1D,2D,3D\}}, \texttt{Glo\-bal\-Max\-Pooling\{1D,2D,3D\}}

\noindent\textbf{Normalization } \texttt{BatchNormalization}, \texttt{GroupNorma\-li\-za\-tion}, \texttt{LayerNormalization}

\noindent\textbf{Arithmetic } \texttt{Add}, \texttt{Average}, \texttt{Subtract}, \texttt{Multiply}, \texttt{tf.mat\-mul}, \texttt{tf.reduce\_mean}, \texttt{tf.reduce\_sum}

\noindent\textbf{Recurrent } \texttt{GRU}, \texttt{LSTM}, \texttt{SimpleRNN}

\noindent\textbf{Shape Adjustment } \texttt{Flatten}, \texttt{Permute}, \texttt{Reshape}, \texttt{Up\-Sampling\{1D,2D,3D\}}, \texttt{Cropping\{1D,2D,3D\}}, \texttt{tf.re\-shape}, \texttt{tf.split}, \texttt{tf.transpose}

\noindent\textbf{Misc. } \texttt{Concatenate}, \texttt{ZeroPadding\{1D,2D,3D\}}, \texttt{Input\-Layer}
}

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

autoinit suggests new default hyperparameter values --> this suggests the old parameters were compensating for incorrect init

should accelerate model development in the future

doesn't have to be the total optimal in every case, but it is a solid default setting that has good motivation behind it

Batchnorm has some good properties, some bad properties.  AutoInit may help to ease the transition away from using bn since it is compatible in both cases.

==> sections/domain_details.tex <==
\section{Experiment domain details}
\label{sec:experiment_domain_details}

% This section describes the experimental setups for each domain in greater detail.

% \subsection{MNIST}

% Models evolved for MNIST were trained for five epochs using the Adam optimizer and batch size 128 \cite{kingma2014adam}.  The initial learning rate is an evolved hyperparameter chosen on a log scale between 0.0001 and 0.01.  No data augmentation was applied to the images.



% \subsection{Omniglot}

% Models were trained for three epochs during evolution, with 1000 iterations per epoch.  No data augmentation is applied to the images.  The initial learning rate is an evolved hyperparamter chosen on a log scale between 0.0001 and 0.001.  


% The learning rate then decays as $\texttt{learning\_rate} = 0.1^{\texttt{epoch}/10}*\texttt{initial\_learning\_rate}$ during training.



% \subsection{PMLB (Adult)}

% The evolved models are trained for 25 epochs with the Adam optimizer \cite{kingma2014adam}.  The batch size is 32.  The initial learning rate is an evolved hyperparameter chosen on a log scale between 0.0001 and 0.01.  No data augmentation was used.
%https://github.com/EpistasisLab/pmlb/blob/master/datasets/adult/metadata.yaml


% \subsection{Wikipedia Toxicity}

% The models are trained with the Adam optimizer \cite{kingma2014adam} for three epochs with a batch size of 128.  The initial learning rate is an evolved hyperparameter chosen on a log scale between 0.0001 and 0.01.  Input tokens are capped at a maximum sentence length of 220.


% \subsection{Oxford 102 Flower}

% The model is optimized with stochastic gradient descent with Nesterov momentum 0.9.  The learning rate is an evolved hyperparameter chosen on a log scale between 0.0001 and 0.1.  Another evolved hyperparameter, \texttt{weight\_decay\_to\_lr\_ratio}, is evolved on a log scale between $10^{-7}$ and $10^{-3}$, and then weight decay (as an L2 loss) of $\texttt{weight\_decay\_to\_lr\_ratio} * \texttt{learning\_rate}$ is applied to all weights and biases.  During training, a batch size of 8 is used, and training progresses for 30 epochs.

% Images are augmented to improve generalization performance.  Images are randomly flipped horizontally, are rotated up to 40 degrees, shifted up/down and left/right up to 20\%, and shear intensity and zoom range are both up to 20\%.

% To save compute resources, training ends early if validation accuracy does not improve for ten consecutive epochs.

% \subsection{ChestX-ray14}

% The ChestX-ray14 dataset contains 112,120 high resolution RGB frontal chest X-ray images \cite{wang2017chestx}.  For each image, the task is to identify the presence or absence of 14 different diseases: some X-rays can have multiple diseases, while others are disease-free.  This dataset naturally lends itself to a multitask learning setup, where there are 14 binary classification tasks associated with each iamge.  The dataset is divided into a 70\%/10\%20\% training/validation/testing split.  The metric used to evaluate networks is the average area under the ROC curve for all 14 tasks (AUROC).  Because many approaches in this task use ImageNet pretrained models, a common preprocessing step which is used here is to resize all images to be 224x224 \cite{deng2009imagenet, wang2017chestx}.

% Models are trained for four epochs.  The models are optimized with Adam \cite{kingma2014adam}.  The initial learning rate is an evolved hyperparameter chosen on a log scale between 0.0001 and 0.001, and it decreases by a factor of 0.1 if the validation loss has not improved for three epochs.  The learning rate decreases in this way at most two times during training.  


% The batch size is one.  The number of training samples is reduced to 20,000 to speed up training.  These samples are randomly selected by stratified sampling.  Let the ratio of positive and negative samples in the dataset be $r_p$ and $r_n$, respectively.  Positive samples are sampled at a rate of $e^{r_p / 0.6} / (e^{r_p / 0.6} + e^{r_n / 0.6})$ while negative samples are sampled at a rate of $e^{r_n / 0.6} / (e^{r_p / 0.6} + e^{r_n / 0.6})$.  This induces a minor bias towards a slightly more balanced dataset, without entirely abandoning the original data distribution.



==> sections/evolved_models.tex <==
\section{Evolved models}
\label{sec:evolved_models}


This section includes visualizations of models evolved for different tasks.  The visualizations illustrate the flexibility of AutoInit.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{network_visualizations/mnist.pdf}
%     \caption{MNIST}
%     \label{fig:mnist}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[height=0.95\textheight]{network_visualizations/omniglot.pdf}
%     \caption{Omniglot}
%     \label{fig:omniglot}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{network_visualizations/pmlb.pdf}
%     \caption{PMLB (Adult)}
%     \label{fig:pmlb}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{network_visualizations/textclassifier.pdf}
%     \caption{Wikipedia Toxicity}
%     \label{fig:textclassifier}
% \end{figure}




==> sections/related_work.tex <==

\section{Related Work}
\label{sec:related_work}

Weight initialization strategies attempt to solve the following fundamental problem: How should weights be initialized so that the neural network does not suffer from vanishing or exploding signals? This section briefly reviews research in this area,
with a more extensive survey in Appendix \ref{ap:related_work_extended}.

Many early contributions stabilized signal propagation in feedforward and convolutional networks, but only when used with specific activation functions \cite{glorot2010understanding, lecun2012efficient, he2015delving}.  After the introduction of residual networks \citep[ResNets;][]{he2016deep, he2016identity}, new weight initialization schemes were developed to account for shortcut connections and various types of residual branches, but these approaches similarly imposed design constraints like requiring specific block structures and activation functions \cite{taki2017deep, zhang2019fixup, arpit2019initialize}.  Data-dependent weight initializations rely on empirical variance estimates derived from the data in order to be model-agnostic \cite{krahenbuhl2015data}.  However, these approaches introduce a computational overhead \cite{mishkin2015all} and suffer when the network is very deep \cite{zhang2019fixup}.

Thus, previous techniques solved the initialization problem for networks with specific activation functions, topologies, and layer types. In contrast, AutoInit does not impose design constraints or incur a parameter overhead \cite{dauphin2019metainit, zhu2021gradinit} and is therefore a good starting point especially in new settings. 




